Monte Carlo Planning in Hybrid Belief POMDPs

Real-world problems often require reasoning about hybrid beliefs, over both discrete and continuous random variables. Yet, such a setting has hardly been investigated in the context of planning. Moreover, existing online Partially Observable Markov Decision Processes (POMDPs) solvers do not support hybrid beliefs directly. In particular, these solvers do not address the added computational burden due to an increasing number of hypotheses with the planning horizon, which can grow exponentially. As part of this work, we present a novel algorithm, Hybrid Belief Monte Carlo Planning (HB-MCP) that utilizes the Monte Carlo Tree Search (MCTS) algorithm to solve a POMDP while maintaining a hybrid belief. We illustrate how the upper confidence bound (UCB) exploration bonus can be leveraged to guide the growth of hypotheses trees alongside the belief trees. We then evaluate our approach in highly aliased simulated environments where unresolved data association leads to multi-modal belief hypotheses.

==> old.tex <==
%Since this is not the main focus of our paper, here we assume that all observed
%instances are (possibly ambiguous) landmarks that exist in the prior belief.

To reason about absent observations, we introduce an association-dependent
observation model,
\begin{equation} \label{def: obs model}
    \mathbb{P}( z_{t}\mid X_{t} ,\beta _{t}).
\end{equation}
Generally, each observation may include multiple instances (e.g. multiple
landmarks), so that $z_t=\left[z_t^1,...,z_t^L\right]$ represents a set of observations
(such as bearing-range or features within an image frame). As all landmarks are
known a-priori, the observation set has a constant size of the landmark
cardinality, $L$. However, usually not all landmarks can be observed at a single
time step, as some may be out of the agent's sensing range. Thus, with slight
abuse of notation, we also allow an observation realization to be empty, denoted as
$z_t^i=\o$.

The intuition behind the association-dependent model is quite simple; For the
clarity, we assume a perfect observation model in the sense that if a landmark
is within the sensing range, an observation of that instance would be obtained.
Under this assumption, the likelihood of obtaining an empty observation, given
that the landmark is within the agent's sensing range, is 0. However, obtaining
an empty observation given that the landmark is located outside of the sensing
range, is 1. 

Using the association dependent model, we update the posterior weights by
sampling states from the propagated distribution, and apply them to equation
\eqref{eq: recursive weight update}. In the considered data-association
scenario, weights are updated according to,
\begin{equation} \label{eq: DA weight update}
    \omega_t^{i,j} = \tilde{\zeta} _{t}^{j\mid i} \omega _{t-1}^{i},
\end{equation}
where,
\begin{align}
    \tilde{\zeta} _{t}^{j\mid i} &= \frac{\zeta _{t}^{j\mid i}}{\sum_i \zeta _{t}^{j\mid i} \omega_{t-1}^i }, \label{normalized_weights} \\ 
    \zeta _{t}^{j\mid i} &= \int _{X_{t}}\mathbb{P}( z_{t} \mid X_{t} ,\beta _{t})\mathbb{P}( \beta _{t} \mid X_{t})\mathbb{P}( X_{t-1} \mid \beta _{0:t-1} ,H_{t}^-). \notag
\end{align}
The latter is obtained by marginalizing $\zeta_t^{i\mid j}$ over the states followed by a
chain-rule.
This procedure accounts for negative information within the belief update. 

\MB{\eqref{eq: recursive weight update}. We may further simplify this expression
by exposing the associations described by $\beta^{i,j}_{t}$ and assuming
conditional independency of an observation given the state variables, to a
product of observation models, $\prod^{I}_{i=1}\mathbb{P}( z_{i, t} \mid
x^{i,j}_{t}, l^{i,j}_{t})$. We denote $x^{i,j}, l^{i,j}$ to relate the specific
state variables to $\beta^{i,j}$. In this setting, the length of the
post-processing observation, $z_{1:I,t}$ represents the number of observed
instances at the current time step. To support no-observations, we extend the
observation received to be at the length of all past landmarks. The gap between
the original observation vector and the new one is filled with an $\o$
indicator,
\begin{equation}
    \mathbb{P}( z_{raw, t} \mid X_{t} ,\beta _{t}) = \mathbb{P}( z_{1:I,t}, z_{I+1:L,t}=\o \mid X_{t} ,\beta _{t}).
\end{equation}
Note that the last step does not add any new information, to what was already
known in \eqref{def: obs model}. We model $\mathbb{P}(z_{i,t}=\o
\mid x^{i,j}_{t}, l^{i,j}_{t})$ as an uninformative, uniform distribution. Last,
we compute $\zeta_t^{i|j}$ apply the result to the weight calculation \eqref{eq: recursive weight update},
\begin{equation}
    \zeta_t^{i|j} = \int_{X_{t}} \prod_{i=1}^{|L|} \mathbb{P}(z_{i,t} \mid X^{i,j}_{t}) \mathbb{P}(\beta^i_{t}\mid X_{t}) \mathbb{P}(X_{t} \mid \beta^{j}_{0:t-1}) \\
\end{equation}
Approximating via state samples, every $\o$ observation degenerates to
the empirical ratio of state-landmark pairs that are within range of the sensor
to the total number of samples,
\begin{gather}
    \int_{X_t} \mathbb{P}(z_{i,t}=\o  \mid X^{i,j}_{t}) \mathbb{P}(\beta^i_{t}\mid X^{i,j}_{t}) \mathbb{P}(X_{t} \mid \beta^{j}_{0:t-1}) \\ \notag
    = c \cdot \mathbb{E}[\mathbb{P}(\beta^i_t \mid X^{i,j}_{t})] \approx \frac{n_{d(x,l)\in FOV}}{n_X}
\end{gather} }


%\begin{table*}[t]
%    \begin{center} \label{table: DA}
%    \begin{tabular}{ |c|c|c|c|c| } 
%        \hline
%        Received observation & Hypothesis $\beta^{i,j}$ assume $(x^{i,j},l^{i,j})$
%       within FOV & Actual sample, $(x^{i,j},l^{i,j})$, within FOV &
%       $\mathbb{P}(z_{i,t}  \mid X^{i,j}_{t}, \beta^{i,j})$ & $\mathbb{P}(\beta^{i,j} \mid X^{i,j})$ \\
%        \hline
%        yes & yes & yes & $\mathcal{N}(\cdot,\cdot)$ & 1  \\
%        \hline
%        yes & yes & no & $\mathcal{N}(\cdot,\cdot)$ & 0 \\
%        \hline
%        no & no & no & 1 & 1 \\ 
%        \hline
%        no & no & yes & 1 & 0 \\
%        \hline
%        yes & no & yes & 1 & 0 \\
%        \hline
%        yes & no & no & 0 & 1 \\
%        \hline
%        no & yes & no & 1 & 0 \\ 
%        \hline
%        no & yes & yes & 0 & 1 \\ 
%        \hline
%    \end{tabular}
%    \end{center}
%    \end{table*}



\MB{
\textbf{Trace estimation.} [consider moving to the implementation section] Trace estimation of some covariance matrix, $\Sigma$,
can be written in terms of the expected distance between the state and the mean,
$\mu$,
\begin{equation}
    trace(\Sigma) = \mathbb{E}_{X}[(X-\mu)^{T}(X-\mu)],
\end{equation}
which can be estimated by first estimating the mean, then using a new set of
samples to compute the expected distance of each sample to the mean. Using
\improvedMCTS, we have only iterative access to the full posterior belief, thus we
store samples from past planning iterations, as described in section
\ref{sec:improvedMCTS}. }

\begin{figure*}[t]
	\centering
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{figs/ambiguous_matrix.png}
		\caption{} 
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{figs/kidnapped.png}
		\caption{} 
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{figs/narrow_pass.png}
		\caption{} 
	\end{subfigure}
	\vskip\baselineskip
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{figs/env_matrix.png}
		\caption{} 
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{figs/env_kidnapped.png}
		\caption{} 
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth]{figs/env_narrow_pass.png}
		\caption{} 
	\end{subfigure}
	\vskip\baselineskip
	\caption{An illustration of the environment being used in our experiments. (a) Shows a trajectory obtained using \vanillaMCTS. (b) A similar trajectory obtained using \improvedMCTS. Depending on the environment, both algorithms may perform equally well.}
	\label{fig:aliasedRoomMap}
\end{figure*} 



\textbf{Uncertainty criteria.} \MB{add refs} There exists an abundance of
uncertainty measures in the literature, see e.g. \MB{\cite{Palaced22tor}} for a
review in the context of active SLAM. Here we discuss only a small, but widely
used subset, devoted to motivating our selection of $\mathcal{A}$-optimality
criteria specifically to multi-hypotheses scenarios. Information-theoretic
functions (such as entropy and information gain), are commonly associated with
Gaussian distributions or discrete variables such as occupancy grid maps. These
functions are most suitable when the distance between different hypotheses is
irrelevant since their value does not depend on the metric distance. In the
context of our interest, for example, estimation of the agent pose (active
localization), locating an object or a group of landmarks, the distance between
plausible points in the distribution is highly relevant, as it may profoundly
affect the motion plan of the agent, whereas two adjacent or highly overlapping
hypotheses might have a negligible effect of the optimal plan.

The second group of common estimators is based on the optimal theory design (e.g.,
$\mathcal{D}$-optimality), which are widely used for Gaussian distributions.
This group of reward functions requires access to the eigenvalues computed from
the covariance matrix of all variables. However, in the non-parametric and/or
hybrid case, the eigenvalues and the covariance matrix are extremely difficult to
estimate in a high-dimensional setting, which precludes most of them from being
practical for online planning.

Nonetheless, the $\mathcal{A}$-optimality, which incorporates the trace of the
covariance matrix can easily be estimated directly from state samples, without
any knowledge of the eigenvalues or covariance matrix. Furthermore, the trace
captures the statistical dispersion of states, which avoids the
distance invariance of information-theoretic functions. Additionally, the
computational complexity of the trace estimation is linear with the number of
state samples, whereas information-theoretic estimators are at least quadratic,
see e.g. \cite{Boers10fusion}.

\textbf{Trace estimation.} Trace estimation of some covariance matrix, $\Sigma$,
can be written in terms of the expected distance between the state and the mean,
$\mu$,
\begin{equation}
    trace(\Sigma) = \mathbb{E}_{X}[(X-\mu)^{T}(X-\mu)],
\end{equation}
which can be estimated by first estimating the mean, then using a new set of
samples to compute the expected distance of each sample to the mean. Using
\improvedMCTS, we have only iterative access to the full posterior belief, thus
we store samples from past planning iterations, as described in section
\ref{sec:improvedMCTS}.



% unbiasdness of weight values

\begin{equation}
	\mathbb{E}_{\mathbb{P}}[\!\!\sum_{\substack{
		k=1 \ s.t. \\
		j(k)=j^\star
		}}^{\left|j^\star\right|} \! \! \!\!  \hat{\omega}_t^j]=\sum_{k=1}^N \frac{1}{N}\mathbb{E}_{\mathbb{P}}[\mathbf{1}_{ \beta=\beta_t^{j^{\!\star}}}]
	= \mathbb{P}(\beta^{j}_t\mid H_t) \!= \omega_t^j.
\end{equation}
